On the Generalizability and Predictability of Recommender Systems

While other areas of machine learning have seen more and more automation, designing a high-performing recommender system still requires a high level of human effort. Furthermore, recent work has shown that modern recommender system algorithms do not always improve over well-tuned baselines. A natural follow-up question is, "how do we choose the right algorithm for a new dataset and performance metric?" In this work, we start by giving the first large-scale study of recommender system approaches by comparing 18 algorithms and 100 sets of hyperparameters across 85 datasets and 315 metrics. We find that the best algorithms and hyperparameters are highly dependent on the dataset and performance metric, however, there are also strong correlations between the performance of each algorithm and various meta-features of the datasets. Motivated by these findings, we create RecZilla, a meta-learning approach to recommender systems that uses a model to predict the best algorithm and hyperparameters for new, unseen datasets. By using far more meta-training data than prior work, RecZilla is able to substantially reduce the level of human involvement when faced with a new recommender system application. We not only release our code and pretrained RecZilla models, but also all of our raw experimental results, so that practitioners can train a RecZilla model for their desired performance metric: https://github.com/naszilla/reczilla.

==> tables/overall_ranking.tex <==
\begin{table}[]
\centering
\small
\caption{Some algorithms perform better than others over all datasets and metrics, however no algorithm dominates all others. This table shows the average rank of each algorithm over all datasets and metrics evaluated in our experiments.\label{tab:overall-alg-ranking}}
\begin{tabular}{@{}lc@{}}
\toprule
Alg. & Avg. Rank\\ \midrule
Item-KNN          & 4.4  \\ 
SVD               & 6.2  \\
User-KNN          & 6.2  \\
SLIM-BPR          & 6.3  \\
MF-FunkSVD        & 6.4  \\
iALS              & 6.5  \\
NMF               & 6.6  \\
P3alpha           & 6.8  \\
MF-BPR            & 7.2  \\
RP3beta           & 7.4  \\
MF-AsySVD         & 7.5  \\
EASE-R            & 8.1  \\
Slime-Elastic-Net & 9.4  \\
TopPop            & 10.2 \\
CoClustering      & 11.8 \\
Random            & 12.0 \\
GlobalEffects     & 12.3 \\
SlopeOne          & 13.8 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_2.tex <==

\begin{table}
\caption{The performance of each rec-sys algorithm varies depending on the dataset and evaluation metric. Each row corresponds to a different metric, precision (PREC) or NDCG, at a particular cutoff. Each algorithm (columns) are ranked according to each metric, values show the ``min/max (mean)'' rank over all datasets for which at least 10 algorithms produced a result (59 out of 89 datasets). Maximum rank is 18, and lower rank indicates better performance. \label{tab:alg-ranks}}
\small
\begin{tabular}{lllllllll}
\toprule
 & \rot{Item-KNN} & \rot{User-KNN} & \rot{P3alpha} & \rot{MF-BPR} & \rot{iALS} & \rot{SLIM-BPR} & \rot{TopPop} & \rot{Random} \\
\midrule
NDCG@1       &      1/4 (1.5) &    2/15 (10.8) &    1/12 (3.6) &  1/15 (10.1) &  1/17 (7.1) &     1/11 (4.0) &   2/17 (9.7) &  10/18 (14.8) \\
% NDCG@2       &     1/10 (1.8) &     2/16 (9.0) &    1/14 (4.0) &  2/15 (10.6) &  1/17 (7.3) &     1/12 (4.2) &  3/17 (10.3) &  10/18 (15.2) \\
NDCG@5       &     1/11 (2.2) &     1/14 (7.2) &    1/14 (3.9) &  3/16 (11.3) &  2/17 (7.1) &     1/12 (4.2) &  1/17 (10.4) &  10/18 (15.4) \\
NDCG@10      &     1/11 (2.2) &     1/13 (6.6) &    1/14 (4.3) &  2/16 (11.2) &  1/17 (7.0) &     1/13 (4.8) &  1/17 (10.2) &  10/18 (15.4) \\
NDCG@50      &     1/11 (2.8) &     1/15 (5.7) &    1/14 (4.8) &  2/15 (11.6) &  1/17 (6.3) &     1/13 (5.9) &   1/16 (9.4) &   9/18 (15.4) \\
PREC@1  &      1/4 (1.5) &    2/15 (10.8) &    1/12 (3.6) &  1/15 (10.1) &  1/17 (7.1) &     1/11 (4.0) &   2/17 (9.7) &  10/18 (14.8) \\
% PREC@2  &     1/11 (1.9) &     2/15 (8.2) &    1/14 (3.9) &  2/15 (10.5) &  1/17 (7.2) &     1/12 (3.8) &  1/17 (10.2) &  10/18 (15.2) \\
PREC@5  &     1/11 (2.5) &     1/14 (5.9) &    1/13 (4.1) &  1/15 (10.7) &  1/17 (6.9) &     1/13 (4.6) &  1/17 (10.2) &  10/18 (15.3) \\
PREC@10 &     1/11 (2.8) &     1/12 (4.9) &    1/13 (4.5) &  1/15 (10.7) &  1/17 (6.1) &     1/12 (5.2) &  1/16 (10.0) &  10/18 (15.4) \\
PREC@50 &     1/12 (4.1) &     1/12 (4.1) &    1/16 (5.5) &  1/15 (10.9) &  1/17 (5.1) &     1/13 (6.9) &   1/16 (8.7) &   9/18 (15.3) \\
% HIT_RATE@1   &      1/4 (1.5) &    2/15 (10.8) &    1/12 (3.6) &  1/15 (10.1) &  1/17 (7.1) &     1/11 (4.0) &   2/17 (9.7) &  10/18 (14.8) \\
% HIT_RATE@2   &     1/11 (1.9) &     2/15 (8.2) &    1/14 (3.9) &  2/15 (10.5) &  1/17 (7.2) &     1/12 (3.8) &  1/17 (10.2) &  10/18 (15.2) \\
% HIT_RATE@5   &     1/11 (2.5) &     1/14 (5.9) &    1/13 (4.1) &  1/15 (10.7) &  1/17 (6.9) &     1/13 (4.6) &  1/17 (10.2) &  10/18 (15.3) \\
% HIT_RATE@10  &     1/11 (2.8) &     1/12 (4.9) &    1/13 (4.5) &  1/15 (10.7) &  1/17 (6.1) &     1/12 (5.2) &  1/16 (10.0) &  10/18 (15.4) \\
% HIT_RATE@50  &     1/12 (4.1) &     1/12 (4.1) &    1/16 (5.5) &  1/15 (10.9) &  1/17 (5.1) &     1/13 (6.9) &   1/16 (8.7) &   9/18 (15.3) \\
% MAP@1        &      1/4 (1.5) &    2/15 (10.8) &    1/12 (3.6) &  1/15 (10.1) &  1/17 (7.1) &     1/11 (4.0) &   2/17 (9.7) &  10/18 (14.8) \\
% MAP@2        &      1/8 (1.6) &     2/16 (9.2) &    1/14 (3.8) &  2/15 (10.5) &  1/17 (7.2) &     1/12 (4.0) &  2/17 (10.2) &  10/18 (15.2) \\
% MAP@5        &     1/11 (2.1) &     2/14 (7.7) &    1/14 (3.8) &  2/15 (11.2) &  1/17 (7.3) &     1/12 (4.2) &  3/17 (10.5) &  10/18 (15.4) \\
% MAP@10       &     1/11 (2.0) &     1/14 (7.4) &    1/14 (4.1) &  2/16 (11.4) &  1/17 (7.3) &     1/12 (4.2) &  1/17 (10.4) &  10/18 (15.4) \\
% MAP@50       &     1/11 (2.2) &     1/14 (7.1) &    1/14 (4.2) &  2/16 (11.5) &  1/17 (7.2) &     1/13 (4.4) &  1/17 (10.0) &  10/18 (15.5) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_3_all_ranks.tex <==
\begin{table}
\caption{The relative performance of each rec-sys algorithm depends on the dataset and metric. This table shows the mean, min (best) and max (worst) rank achieved by all algorithms over all 85 datasets, over 10 accuracy and hit-rate metrics at all cutoffs tested. This includes metrics NDCG, precision, recall, Prec.-Rec.-Min-density, hit-rate, F1, MAP, MAP-Min-density, ARHR, and MRR.\label{tab:overall-ranks}}
\tabcolsep3pt 
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllllllllllllllll}
\toprule
Rank & \rot{Item-KNN} & \rot{SLIM-BPR} & \rot{SVD} & \rot{P3alpha} & \rot{iALS} & \rot{User-KNN} & \rot{NMF} & \rot{RP3beta} & \rot{EASE-R} & \rot{MF-FunkSVD} & \rot{SLIM-ElasticNet} & \rot{MF-AsySVD} & \rot{MF-BPR} & \rot{TopPop} & \rot{CoClustering} & \rot{GlobalEffects} & \rot{SlopeOne} & \rot{Random} \\
\midrule
mean &        3.4 &        5.0 &   5.7 &       5.7 &    6.0 &        6.2 &   6.4 &       6.7 &      6.7 &          7.5 &                 7.8 &         8.2 &      8.6 &      9.9 &            11.8 &             12.1 &         13.2 &      14.2 \\
min  &              1 &              1 &         1 &             1 &          1 &              1 &         1 &             1 &            1 &                1 &                     1 &               1 &            1 &            1 &                  1 &                   1 &              1 &            2 \\
max  &             17 &             14 &        16 &            17 &         17 &             16 &        15 &            16 &           17 &               16 &                    16 &              15 &           16 &           18 &                 17 &                  18 &             18 &           18 \\
\bottomrule
\end{tabular}
%}
\end{table}
